Low Vibration Closed-Cycle Flow Cryostat for Ion-Cavity Experiments

Cryogenic operation below 10 K suppresses trap-electrode and dielectric heating of trapped ions while cryopumping residual gases to ultra-high vacuum (UHV) without requiring a bakeout. These advantages are particularly important for cavity-integrated ion traps, where nearby dielectric surfaces can increase motional heating and rapid design-build-test iterations benefit from eliminating bakeout cycles. We have developed a custom 4 K cryostat cooled by a ColdEdge Technologies (CET) Stinger closed-cycle $^{4}\text{He}$ flow cryogenic system to study various ion trap optical cavity structures designed to serve as a photonic interconnect between remote, compute-capable trapped $^{171}\text{Yb}^{+}$ ion quantum processors, enabling long baseline entanglement distribution $(>10\text{ km})$. We integrate an Alpine Quantum Technologies (AQT) Paul trap and Fabry-P\'erot optical cavity at the 4 K stage. The cooling capacities of the cryostat 40 K and 4 K stages were measured to be 5 W at 45 K and 0.5 W at 6.1 K. Vibrations of the 4 K stage relative to the optical table are less than $12\text{ nm}_{\text{RMS}}$ in three dimensions, as measured using a Michelson interferometer. An ultra-high vacuum (UHV) is inferred by studying the rate of hydrogen-$\mathrm{Yb}^{+}$ ion collisions. Ion storage times exceeding 5 days without laser cooling have been reported and the position of the trapped ions are reproducible within $\sim10\text{ }\mu\text{m}$ following repeated thermal cycles to room temperature. The uptime of this system is 72 days and offers convenient access to the 4 K stage for in-vacuum maintenance and system modifications. Using this platform, we demonstrate spatial overlap and interaction between a trapped $^{174}\text{Yb}^{+}$ ion and the optical cavity mode on the 1345 nm transition, establishing preliminary experimental validation of the integrated cryogenic ion-cavity structure.

==> Bibliography.tex <==

\vspace*{-1in}

\begin{thebibliography}{99}
\vspace{-.25in}

\setlength{\parskip}{1em}

\bibitem{Agrawal1} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 1.
\bibitem{Bloembergen} N. Bloembergen, {\em Nonlinear Optics} (Benjamin,
Reading, MA, 1977).
\bibitem{Shen} Y.R. Shen, {\em Principles of Nonlinear Optics} (Wiley, New
York, 1984).
\bibitem{Butcher} P.N. Butcher and D.N. Cotter, {\em The Elements of
Nonlinear Optics} (Cambridge University Press, Cambridge, UK, 1990).
\bibitem{Boyd} R.W. Boyd, {\em Nonlinear Optics} (Academic Press, San Diego,
CA, 1992).
\bibitem{Newell} A.C. Newell and J.V. Moloney {\em Nonlinear Optics (Advanced Topics in the Interdisciplinary Mathematical Sciences)} (Westview Press, Boulder, CO, April 1992).
\bibitem{Marcuse} D. Marcuse,{\em Light Transmission Optics} (Van Nostrand
Reinhold, New York, 1982), Chaps. 8 and 12.
\bibitem{Agrawal2} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 2.
\bibitem{Diament} P. Diament, {\em Wave Transmission and Fiber Optics}
(Macmillan, New York, 1990).
\bibitem{Zakharov} V.E. Zakharov and A.Shabat, Sov. Phys. JETP
\textbf{34}, 62 (1972)
\bibitem{Hardin} R.H. Hardin and F.D. Tappert, SIAM
Rev. Chronicle \textbf{15}, 423 (1973).
\bibitem{Fisher} R.A.Fisher and
W.K. Bischel, Appl. Phys. Lett. \textbf{23}, 661 (1973); J. Appl. Phys
\textbf{46}, 4921 (1975).
\bibitem{Cooley} J.W. Cooley and J.W. Tukey,
Math. Comput. \textbf{19}, 297 (1965).
\bibitem{Trebino} R. Trebino, D.J. Kane, "Using phase retrieval to measure
the intensity and phase of ultrashort pulses: frequency resolved optical gating," J. Opt. Soc. Am. B \textbf{10}, 1101 (1993).
\bibitem{Kanejqe} D.J. Kane, R. Trebino, "Characterization of Arbitrary Femtosecond Pulses Using Frequency-Resolved Optical Gating," IEEE J. Quant. Elect. \textbf{29}, 571 (1993).
\bibitem{Kaneoptlett} D.J. Kane, R. Trebino, "Single-shot measurement of the intensity and phase of an arbitrary ultrashort pulse  by using frequency-resolved optical gating," Opt. Lett. \textbf{10}, 1101 (1993).
\bibitem{OShealett}P. O'Shea, M. Kimmel, X. Gu, R. Trebino, "Highly simplified device for ultrashort-pulse measurement," Opt. Lett. \textbf{26}, 932 (2001).
\bibitem{Agrawal3} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 3.
\bibitem{Agrawal4} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 4.
\bibitem{Agrawal10} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 10.
\bibitem{Agrawal7} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 7.
\bibitem{Agrawal6} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 6.
\bibitem{Stolen} R.H. Stolen, E.P. Ippen, and A.R. Tynes,
Appl. Phys. Lett. \textbf{20}, 62 (1972).
\bibitem{Ippen} E.P. Ippen and R.H. Stolen, Appl. Phys. Lett. \textbf{21},
539 (1972).
\bibitem{Smith} R.G. Smith, Appl. Opt. \textbf{11}, 2489 (1972).
\bibitem{Agrawal9} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 9.
\bibitem{Agrawal8} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 8.
\bibitem{hart1} D.L. Hart, Arthur F. Judy, Rajarshi Roy and James W. Beletic, Phys. Rev. E \textbf{57}, 4757 (1998); D.L. Hart, Arthur F. Judy, T.A.B. Kennedy, Rajarshi Roy and K. Stoev, Phys. Rev. A \textbf{50}, 1807 (1994).
\bibitem{ito} K. Ito, {\em Lectures on Stochastic Processes} (Tata Institute of Fundamental Research, Bombay, 1960).
\bibitem{stratanovich} R.L. Stratanovich, {\em Topics in the Theory of Random Noise}, Vols I. and II. (Gordon \& Breach, New York, 1963).
\bibitem{risken} H. Risken, {\em The Fokker-Planck Equation} (Springer-Verlag, Berlin, 1989).
\bibitem{werner2} M.J. Werner and P.D. Drummond, J. Comput. Phys. \textbf{132}, 312 (1997).
\bibitem{drummond1} P.D. Drummond and I.K. Mortimer, J. Comput. Phys. \textbf{93}, 144 (1991).
\bibitem{carter3} S.J. Carter, Phys. Rev. A. \textbf{51}, 3274 (1995).
\bibitem{thompson1} J.R. Thompson and Rajarshi Roy, Phys. Rev. A \textbf{43}, 4987 (1991).
\bibitem{boxmuller} W.H. Press, S.A. Teukolsky, W.T. Vetterling and B.P. Flannery, {\em Numerical Recipes in Fortran: The Art of Scientific Computing} (Cambridge University Press, Cambridge, 1992).
\bibitem{headley} C. Headley, G.P. Agrawal, IEEE J. Quantum Electron. \textbf{QE-31}, 2058 (1995), C. Headley, G.P. Agrawal J. Opt. Soc. Am. B. \textbf{13}, 2170 (1995).
\bibitem{perlmutter1} S.H. Perlmutter, M.D. Levenson, R.M. Shelby and
M.B. Weisman, Phys. Rev. Lett. \textbf{61} 1388, 1988.
\bibitem{abdullaev} F. Kh. Abdullaev, J.H. Hensen, S. Bischoff and M.P. Sorensen, J. Opt. Soc. Am. B. \textbf{15}, 2424 (1998); F. Kh. Abdullaev, J.G. Caputo, and Nikos Flytzanis, Phys. Rev E. \textbf{50}, 1552 (1994).
\bibitem{glenn} William H. Glenn, IEEE J. Quantum Electron. \textbf{QE-25}, 1218 (1989).
\bibitem{Trebinobook} R. Trebino. {\em Frequency-Resolved Optical Gating: The Measurement of Ultrashort Laser Pulses} (Kluwer Academic 2002).
\bibitem{Agrawal} G.P. Agrawal {\em Nonlinear Fiber Optics} (Academic,
San Diego, 2001).
\bibitem{Dudley} J.M. Dudley, X. Gu, L. Xu, M. Kimmel, E. Zeek, P. O'Shea, R. Trebino, S. Coen, R.S. Windeler, "Cross-correlation frequency resolved optical gating analysis of broadband continuum generation in photonic crystal fiber: simulations and experiments," Opt. Express \textbf{10}, 1215 (2002).
\bibitem{Liu1} Q.D. Liu, J.T. Chen, Q.Z. Wang, P.P. Ho, and R.R. Alfano, "Single pulse degenerate-cross-phase modulation in a single-mode optical fiber," Opt. Lett. \textbf{20}, 542 (1995).
\bibitem{Sylvestre} T. Sylvestre, H. Maillotte, E. Lantz, and D. Gindre "Combined spectral effects of pulse walk-off and degenerate cross-phase modulation in birefringent fibers", Journal of Nonlinear Optical Physics and Materials 6, 313-320 (1997).
\bibitem{Liu2} Q.D. Liu, L. Shi, P.P. Ho, R.R. Alfano, R.J. Essiambre, and G.P. Agrawal, "Degenerate cross-phase modulation of femtosecond laser pulses in a birefringent single-mode fiber," IEEE Photon. Tech. Lett. \textbf{9}, 1107 (1997).
\bibitem{Omenetto1} F.G. Omenetto, B.P. Luce, D. Yarotski and A.J. Taylor, "Observation of chirped soliton dynamics at l= 1.55 mm in a single-mode optical fiber with frequency-resolved optical gating," Opt. Lett. \textbf{24}, 1392 (1999).
% 1.55 micron regime - check for more recent papers by Omenetto use both web-sci and inspec
\bibitem{Omenetto2} F.G. Omenetto, Y. Chung, D. Yarotski, T. Shaefer, I. Gabitov and A.J. Taylor, "Phase analysis of nonlinear femtosecond pulse propagation and self-frequency shift in optical fibers," Opt. Commun. \textbf{208}, 191 (2002).
\bibitem{Omenetto3} F.G. Omenetto, J.W. Nicholson, B.P. Luce, D. Yarotski, A.J. Taylor, "Shaping, propagation and characterization of ultrafast pulses in optical fibers," Appl. Phys. B \textbf{70}[Suppl.], S143 (2000).
\bibitem{Nishizawa1} N. Nishizawa and T. Goto, "Experimental analysis of ultrashort pulse propagation in optical fibers around zero-dispersion region using cross-correlation frequency resolved optical gating," Opt. Express \textbf{8}, 328 (2001).
\bibitem{Nishizawa2} N. Nishizawa and T. Goto, "Trapped pulse generation by femtosecond soliton pulse in birefringent optical fibers," Opt. Express \textbf{10}, 256 (2002).
\bibitem{Nishizawa3} N. Nishizawa and T. Goto, "Characteristics of pulse trapping by use of ultrashort soliton pulses in optical fibers across the zero-dispersion wavelength," Opt. Express \textbf{10}, 1151 (2002).
\bibitem{Nishizawa4} N. Nishizawa and T. Goto, "Ultrafast all optical switching by use of pulse trapping across zero-dispersion wavelength," Opt. Express \textbf{11}, 359 (2003).
% All of Nishizawa and Goto papers are related to 1.3 micron experiments and simulations.
\bibitem{Ogawa}, K. Ogawa, M.D. Pelusi, "Characterization of ultrashort optical pulses in a dispersion-managed fiber link using two-photon absorption frequency-resolved optical gating," Opt. Commun. \textbf{198}, 83-87 (2001).
\bibitem{Altes} R.A. Altes, "Detection, estimation, and classification
with spectrograms," J. Acoust. Soc. Am. \textbf{67}(4), 1232 (1980).
\bibitem{Christian} A. Christian Silva, "GRENOUILLE - Practical Issues," unpublished.
\bibitem{Mejia} J. Garduno-Mejia, A.H. Greenaway, and D.T. Reid, "Designer
femtosecond pulses using adaptive optics," Opt. Express \textbf{11}
2030 (2003).
\bibitem{OSheaexpress1} P. O'Shea, M. Kimmel, X. Gu, R. Trebino, "Increased-bandwidth in ultrashort-pulse measurement using an angle-dithered nonlinear-optical crystal," Opt. Express \textbf{7}, 342 (2000).
\bibitem{OSheaexpress2} P. O'Shea, M. Kimmel, R. Trebino, "Increased phase-matching bandwidth in simple ultrashort-laser-pulse measurements," J. Opt. B \textbf{4}, 44 (2002).
\bibitem{Akturk} S. Akturk, M. Kimmel, P. O'Shea, R. Trebino, "Measuring pulse-front tilt in ultrashort pulses using GRENOUILLE", Opt. Express \textbf{11}, 491 (2003).
\bibitem{Blow} K. J. Blow, D. Wood, "Theoretical Description of Transient Stimulated Raman Scattering in Optical Fibers," IEEE J. Quant. Elect. \textbf{25}, 2665 (1989).
\bibitem{Stolen2} R.H. Stolen, J.P. Gordon, W.J. Tomlinson,
J. Opt. Soc. Am. B \textbf{6}, 1159 (1989).
\bibitem{Mamyshev} P.V. Mamyshev and S.V. Chernikov, Sov. Lightwave
Commun. \textbf{2}, 97 (1992).
\bibitem{Headleythesis} C. Headley III, \em{Ultrafast Stimulated Raman
Scattering in Optical Fibers}, Ph.D. Thesis, University of Rochester,
NY (1995).
\end{thebibliography}


==> Dedication.tex <==
%Dedication
\vspace{.65in}

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }

\vspace*{-.85in}


\begin{center}
\large{Dedication}
\end{center}

If needed.


==> Foreword.tex <==
%Foreword

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }

\vspace*{-.85in}

\begin{center}
\large{Foreword}
\end{center}

If needed.

